Atlas: Accelerating Quantum FTQC Compilation with Optimized Algebraic Rotation Synthesis

As fault-tolerant quantum computing emerges, Clifford+T gate basis becomes a popular choice where we need to decompose single-qubit rotation gates into gates in this gate basis. Quantum rotation synthesis may lead to remarkable overhead in quantum circuit compilation. Considering variational quantum eigensolver (VQE) applications as an example, a conventional UCCSD ansatz in quantum chemistry can generate $O(n^4)$ rotations for $n$ qubits. Each optimization iteration updates the rotation angles, making rotation synthesis a recurring cost that can delay the VQE training loop. We identify two sources of delay in rotation synthesis: redundant computation during synthesis and uneven synthesis times that leave workers waiting for slow requests. Atlas addresses these costs with three optimizations: search pruning skips invalid synthesis candidates through statistical inference; adaptive arithmetic avoid unnecessary high-overhead big integer/float arithmetic when decomposing the target rotation gate; batch scheduling fills the gap between the synthesis time of varied rotations. Across various benchmarks, synthesis method, and compilation machines, Atlas can consistently accelerate the rotation synthesis process by up to 12.65x.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
QCOLA exploits spatial and temporal sparsity in LC qubit use to acquire hardware information alongside user execution. Its BE opportunity admission controller selects feasible targets and windows, its observation manager turns fragmented characterization into validated estimates, and its scheduler integration exposes versioned profiles to existing decision processes. The observation manager supports five hardware characteristics; the quantitative evaluation uses coherence-time feedback. These components preserve scheduling objectives and algorithms. The Qonductor integration improves execution fidelity in the completed four-QPU study; its assignment control and waiting-weight sweep show how queue interactions and objective settings affect completion time. The \mbox{Q-BEEP} cases demonstrate that updated profiles can also benefit an unchanged reconstruction procedure.

\section*{Content Generated by AI}
GPT-6 (Codex) assisted with drafting, polishing, and translating the abstract and Sections~\ref{sec:introduction}--\ref{sec:conclusion}, organising references, creating editable conceptual diagrams, and producing reporting and typesetting scripts. Inputs included project code, published sources, and archived simulation outputs. This revision reports the completed four-QPU cohort, 4/8/16-QPU capacity study, and waiting-weight study, and the completed arrival-rate comparison. 

